Learning a Formally Verified Control Barrier Function in Stochastic Environment

Safety is a fundamental requirement of control systems. Control Barrier Functions (CBFs) are proposed to ensure the safety of the control system by constructing safety filters or synthesizing control inputs. However, the safety guarantee and performance of safe controllers rely on the construction of valid CBFs. Inspired by universal approximatability, CBFs are represented by neural networks, known as neural CBFs (NCBFs). This paper presents an algorithm for synthesizing formally verified continuous-time neural Control Barrier Functions in stochastic environments in a single step. The proposed training process ensures efficacy across the entire state space with only a finite number of data points by constructing a sample-based learning framework for Stochastic Neural CBFs (SNCBFs). Our methodology eliminates the need for post hoc verification by enforcing Lipschitz bounds on the neural network, its Jacobian, and Hessian terms. We demonstrate the effectiveness of our approach through case studies on the inverted pendulum system and obstacle avoidance in autonomous driving, showcasing larger safe regions compared to baseline methods.

==> conclusions.tex <==
In this paper, we proposed an algorithmic approach to learn a valid continuous time CBF with formal guarantees in a stochastic environment. The CBF is learned using loss functions that enforce the CBF conditions and the CBF constraint. The effectiveness of our proposed approach is demonstrated using the simulation study on inverted pendulum. In future works, we plan to account for unknown dynamics and perform experiments on robotic systems in real life.

% In this paper, we study the problem of exact verification of CLF/CBF compatibility and synthesis compatible CLF/CBF. 
% We consider a continuous-time stochastic nonlinear control-affine system. 
% We derive the sufficient condition for the safety of SNCBF-based system. 
% We construct a sample-based training framework to train SNCBF and prove the trained SNCBF ensuring efficacy across the entire state space with only a finite number of data points. To summarize, this paper makes the following contributions.

==> introduction.tex <==


In the rapidly evolving landscape of control theory, ensuring safety in real-world applications has emerged as a paramount concern. With the pervasive integration of automated systems such as self-driving cars, the ability to guarantee their safety becomes increasingly critical. Current methods, including traditional optimal control approaches and Hamilton-Jacobi reachability analysis, have been instrumental in addressing safety requirements by casting them as constraints or generating safe controls offline. However, the scalability limitations of these methods, coupled with the challenge of swift reactions in complex environments, underscore the need for alternative approaches to safety assurance.
With the rise in popularity of learning-based methods in control synthesis, learning-based methods have also been used to synthesize controllers for safety-critical tasks. However, most learning-based methods require a significant amount of unsafe interactions to learn a safe controller, which might be costly or impossible to obtain.

One promising avenue in addressing safety concerns is through the utilization of Control Barrier Functions (CBFs) \cite{Ames_2017}\cite{8796030}. CBFs serve as a practical method for synthesizing safe control by acting as a safety filter for potentially unsafe performance controllers. By formulating controllers through Quadratic Programs (QPs), solvable at high frequencies with modern optimization solvers, CBFs have found applications in various safety-critical tasks, including bipedal and quadrupedal locomotion, adaptive cruise control, and multi-agent aerial maneuvers. However, traditional methods for identifying valid CBFs face challenges, particularly with nonlinear or nonconvex constraints, necessitating the exploration of alternative approaches to ensure the efficacy of CBFs in guaranteeing safety.

In recent years, the emergence of neural network-based safety certificate synthesis has garnered considerable attention as a potential solution to the limitations of classical approaches. By parameterizing formulations as neural networks, the need for a mathematical model is circumvented, offering greater flexibility and adaptability in addressing safety specifications. However, this approach introduces its own set of challenges, as neural network-based formulations lack formal guarantees and may not satisfy conditions across the entire state set due to finite training samples. Thus, while neural network-based CBFs hold promise in enhancing safety assurance, further exploration and development are needed to address their current limitations and ensure their applicability in safety-critical systems.

% However, a major caveat of the aforementioned approach is that it requires mathematical knowledge about the system in the form of a model. Since precise mathematical models are not always available due to large complexity of the systems, one needs to consider alternative model-free approaches. Another drawback of the approach is the difficulty in searching for suitable CBFs. In general, one requires to find an appropriate and valid CBF

% In recent year learning based controllers have shown great promise, but there are no safety guarantees, thus making it hard to be applied for safety-critical applications.

%  In recent years, the development of machine learning (ML) has created unprecedented opportunities to control modern autonomous systems with growing complexity.

%  There is some existing work, that synthesises a CBF using neural networks but they lack the completeness guarantees. There is also some work on the synthesis of safe controller using neural network based control barrier certificates (CBC) in discrete time setting along with the completeness guarantee. 

%  In this work, we present a 


%  Ensuring safety is crucial when designing controllers for real-world applications. With the increasing usage of automated systems, e.g., self-driving cars, the ability to guarantee the safety of such systems becomes increasingly important. In optimal control, safety is often ensured by casting the safety requirements as constraints. However, when the optimization problem gets larger, the solution time increases rapidly, limiting its usage for guaranteeing safety in complex environments, which usually requires the control system to react quickly. Recently, Hamilton-Jacobi reachability analysis has been used to generate safe controls. When solved offline, it provides a way to generate safe controls quickly online. However, its usage is greatly limited by the curse of dimensionality. With the rise in popularity of learning-based methods in control synthesis, learning-based methods have also been used to synthesize controllers for safety-critical tasks. However, most learning-based methods require a significant amount of unsafe interactions to learn a safe controller [28], which might be costly or impossible to obtain.

% Another popular method to synthesize safe control is utilizing control barrier functions (CBFs). CBFs can be used as a safety filter for an unsafe performance controller. The controller can be obtained by solving a quadratic program (QP) which can be done at a very high frequency using modern optimization solvers. Given its many advantages, CBFs have been used on many safety-critical tasks, e.g., biped and quadrupedal locomotion on stepping stones [26] [16], adaptive cruise control [2], and multi-agent aerial maneuver [29].

% Although CBF provides a promising direction in safe controller synthesis, we need to have the access to a valid $\mathrm{CBF}$. A common approach to finding a valid CBF is to start with a description of the safe set, usually in the form of state constraints, and find a function that is positive only within the safe set and has the appropriate relative degree with respect to the system dynamics. This method is plausible for simple constraints. However, finding a valid CBF that recovers the entire safe set becomes increasingly challenging as the constraints become nonlinear or nonconvex. To mitigate this issue, work has been done in learning the CBF. In [31], human demonstrations have been used to map the boundaries of the safe set, and a CBF is then learned. This method may not scale to constraints in higher dimensions. Instead of having information on safe set boundaries, work has been done on utilizing expert demonstrations of safe and unsafe trajectories [30]. Additionally, work has been done in learning CBFs using data collected online. In [22], a $\mathrm{CBF}$ is synthesized using only onboard sensors. Recently, work has been done in learning a CBF starting from an initial conservative CBF. In [34], an $\mathrm{HCBF}$ is used to warm start a dynamic program that refines the HCBF to enlarge the recovered safe set. In [12], a learning-based approach is used to learn the difference between a conservative $\mathrm{HCBF}$ and a $\mathrm{CBF}$ that recovers a more significant portion of the safe set.


% Formal verification and synthesis of complex systems against safety specifications is of utmost importance in the field of control theory, especially due to the emergence of safety-critical applications such as autonomous vehicles, drones, robots, medical devices, etc. Methods utilizing control barrier functions (CBFs) provide an effective mechanism to formally generate controllers enforcing the satisfaction of safety specifications. In particular, control barrier functions are real-valued functions defined over the state set of the system. They act as a barrier between the safe and unsafe regions, providing sufficient conditions such that the barrier is never crossed by the closed-loop system trajectories. However, a major drawback of this approach is the difficulty in finding a suitable $\mathrm{CBF}$ especially for large complex systems.

% Neural network-based safety certificate synthesis has gained considerable attention recently (Dawson et al., 2023) since it has great potential to alleviate the issues concerning model-based one. First, neural network training is completely data-driven. Therefore, by parameterizing CBFs as neural networks, one avoids the requirement of a mathematical model. Second, neural networks are capable of approximating any continuous function (Barron, 1994). However, CBFs based on neural networks lack formal guarantees and cannot be applied to safety-critical systems without further verification. This is due to the fact that neural networks are trained on a finite number of samples from the state set, and as a result, the trained networks are not guaranteed to satisfy the required $\mathrm{CBF}$ conditions over the entire state set (i.e. unseen samples from the state set). Therefore, one is required to formally verify the trained CBFs post facto to ensure safety.

\subsection{Related Work}

Barrier certificates for safe control were first proposed in \cite{prajna2007framework}. More recently, CBFs have emerged as promising approaches to safe control, due to their compatibility with a wide variety of control laws. For control systems with polynomial dynamics, CBFs can be synthesized by solving sum-of-squares (SOS) optimization programs \cite{clark2021verification,clark2022semi,kang2023verification,dai2023convex}. 
Polynomial CBFs are limited in applications due to the limitation of the template and function space \cite{anand2023formally}. 
To overcome the shortcomings of CBF synthesis using SOS-based approaches, neural control barrier functions (NCBFs) \cite{dawson2022safe,dawson2023safe,liu2023safe,9993334, dai2023learning}, which represent CBFs using neural networks, are developed.
Recent research shows great promise of neural barrier functions in flexibility in configuring complex environments and potential to scale up. 
NCBFs leverage the universal approximation power of neural networks \cite{tabuada2022universal,hornik1989multilayer,csaji2001approximation}, facilitating the CBF synthesis.
A class of recent neural barrier certificate is to construct a nominal control policy and prove that it satisfies the NCBF constraints, including SMT-based methods~\cite{zhao2020synthesizing,abate2021fossil,abate2020formal}, mixed integer programs \cite{zhao2022verifying} and nonlinear programs \cite{NEURIPS2023_120ed726}.
\textcolor{blue}{[details on related work on neural control barrier certificate]}
Existing works focused on certificating deterministic systems and joint synthesis of safe control policy \cite{jin2020neural}. However, safety verification of stochastic systems are less explored. 

% \cite{10.1145/3447928.3456638} \cite{10066195} \cite{10.1007/978-3-030-72016-2_20} \cite{9157966} \cite{9990576}

\subsection{Contributions}
The main contributions of our work are:
We propose a training framework to synthesize provably correct Control Barrier Functions (CBFs) parameterized as neural networks for continuous-time, stochastic systems eliminating any need for post hoc verification. Our methodology establishes completeness guarantees by deriving a validity condition, ensuring efficacy across the entire state space with only a finite number of data points. We train the network robustly, by enforcing Lipschitz bounds on the neural network, its Jacobian and Hessian terms. Validation of our approach is demonstrated through simulation experiments conducted on an inverted pendulum.

\subsection{Organisation}
The rest of this paper is organized as follows. Preliminaries explaining the concept of control barrier functions (CBFs) and safety filter designs are introduced in Section \ref{section: Background}. Problem formulation is discussed in Section \ref{section: Problem Formulation}. The method proposed to synthesize the CBFs using neural networks, the construction of loss functions and algorithm to train it, is discussed in Section \ref{section: Method}. The simulation results will be discussed in Section \ref{section: Simulation}. Finally, we present our conclusion in Section \ref{section: Conclusions}. 



% $<.\:,\:.>$ denotes the inner product of two vectors.
% $\hat{i}$ and $\hat{j}$ stands for unit vectors along x-axis and y-axis respectively. The units used in the simulations are SI units.

==> method.tex <==
In this section, we propose an algorithmic approach to solve the problem formulated in Section \ref{section: Problem Formulation}. The structure of this section is as follows. First, we describe our proposed framework for the Neural CBF  and then we talk about training process for the same. 

\subsection{Structure of the Neural Network}
\label{subsection: nn_structure}
% After establishing the problem framework in Section \ref{section: Problem Formulation}, the task at hand involves the estimation of the continuously differentiable function $h(x)$, denoted as $\tilde{h}(x \mid \theta)$, through the application of a deep neural network (DNN). Here, $\theta$ signifies the weights associated with the DNN.

In order to maintain the required continuity, we necessitate that $\tilde{h}(x \mid \theta)$ also be continuously differentiable concerning the input $x$. To achieve this, we adopt a deep differential network employing smooth activation functions, as elucidated in detail in \cite{lutter2019deep}. The deep differential network is equipped with three forward paths – one akin to standard fully-connected DNNs, the second to computing the Jacobian and the third to compute the Hessian of the DNN concerning its input. The direct output of the Jacobian and Hessian, rather than undergoing an additional numerical differentiation pass, enhances computational efficiency. The structure of a single layer within a deep differential network is defined as:

\begin{equation}
    \left(\frac{\partial^2 \overline{y}}{\partial y^2},\frac{\partial \overline{y}}{\partial y}, \overline{y}\right)=\ell(y)
\end{equation}

Here, $y \in \mathbb{R}^{n_{i} \times 1}$ represents the layer input, $\overline{y} \in \mathbb{R}^{n_{o} \times 1}$ signifies the layer output, and the layer is denoted as $\ell: \mathbb{R}^{n_{i} \times 1} \rightarrow\left(\mathbb{R}^{n_{o} \times n_{i}}, \mathbb{R}^{n_{o} \times 1}\right)$. The Jacobian computation is expressed as:

\begin{equation}
    \frac{\partial \overline{y}}{\partial y}=\operatorname{diag}\left(\mathbf{g}^{\prime}(\mathbf{a})\right) \mathbf{\theta}
\end{equation}

Here, $\mathbf{\theta} \in \mathbb{R}^{n_{o} \times n_{i}}$ denotes the layer weights, $\mathbf{g}: \mathbb{R}^{n_{o} \times 1} \rightarrow \mathbb{R}^{n_{o} \times 1}$ represents the activation function, $\mathbf{g}^{\prime}(\cdot)$ signifies the derivative of the activation function, and $\mathbf{a}=\mathbf{\theta} y+$ bias.

\subsection{Learning CBF with formal guarantees}
In this section, we discuss the procedure to learn the CBF $ \tilde{h}(x \mid \theta)$  while ensuring the satisfaction of the validity condition \eqref{eq: completeness_condition} such that the trained CBF and controller satisfy conditions \eqref{eq:setc1},\eqref{eq:setc2},\eqref{eq: lie_derivative} over the entire state set $X$. To do this, one requires Lipschitz continuity of $\tilde{h}(x \mid \theta)$ and its derivative $\frac{\partial \tilde{h}\left(x_{i} \mid \theta\right)}{\partial x}$. The function $\tilde{h}(x \mid \theta)$ is Lipschitz continuous with a bound $\mathcal{L}_{h}$ if:

\begin{equation}
    \left\|\tilde{h}(x \mid \theta)-\tilde{h}(y \mid \theta)\right\| \leq \mathcal{L}_{h}\|x-y\|, \quad \forall x, y \in \mathbb{R}^{n}    
\end{equation}

Now, \cite{pauli2021training} gives a framework to train multi-layer NNs while at the same
allowing to enforce a desired Lipschitz bound on the NN at all times during training.
More specifically, it provides an optimization scheme based on the Alternating Direction Method of Multipliers (ADMM) that minimizes not only the training loss of an NN but also its Lipschitz constant resulting in a semidefinite programming based training procedure. 

To find the weights $\theta$, we would now need to decide the loss functions. A widely used approach \cite{qin2022sablas} is to learn a valid CBF with ground truth labels by utilizing the properties in (5) and write the loss functions for learning $\theta$ as

\begin{equation}
    \begin{aligned}
        & \mathcal{L}_{s}(\theta, \eta)=\frac{1}{N} \sum_{x_{i} \in \mathcal{X}_{s}} \max \left(0,-\tilde{h}\left(x_{i} \mid \theta\right) - \eta \right), \\
        & \mathcal{L}_{u}(\theta, \eta)=\frac{1}{N} \sum_{x_{i} \in \mathcal{X}_{u}} \max \left(0, \tilde{h}\left(x_{i} \mid \theta\right)- \eta\right)
    \end{aligned}
\end{equation}

with $\mathcal{L}_{s}$ representing the loss for safe states, $\mathcal{L}_{u}$ representing the loss for unsafe states, $\mathcal{X}_{s}$ being the dataset containing safe states, $\mathcal{X}_{u}$ being the dataset containing unsafe states. We can see that for a safe state, $\mathcal{L}_{s}$ is only non-zero when the estimated $\tilde{h}(x \mid \theta)$ is negative. For unsafe states, $\mathcal{L}_{u}$ is only non-zero when the estimated CBF is positive. Thus, in both cases, only when the sign of the estimated CBF is wrong will there be a non-zero loss; otherwise, the loss is zero. 

In addition to the CBF losses, we add another loss corresponding to the CBF constraint in \eqref{eq: lie_derivative} to ensure the ability to generate safe control actions

\begin{equation}
    \begin{aligned}
        \mathcal{L}_{\nabla \mathbf{h}}(\theta, \eta)= & \frac{1}{N} \sum_{x_{i} \in \mathcal{X}} \max \left(0, -\frac{\partial \tilde{h}\left(x_{i} \mid \theta\right)}{\partial x} (f(x_{i})+g(x_{i}) u(x_{i})  \right. \\
        & \left. - \frac{1}{2}tr(\sigma^\intercal \frac{\partial^2 \tilde{h}\left(x_{i} \mid \theta\right)}{\partial x^2} \sigma)  - \alpha\left(\tilde{h}\left(x_{i} \mid \theta\right)\right)- \eta \right)
    \end{aligned}
\end{equation}

We will defer the discussion of the learning procedure to Section \ref{training}.

Using the terms defined above, the final loss function is given by

\begin{equation}
    \mathcal{L}_{\theta}(\theta)=\mathcal{L}_{s}+\lambda_{1} \mathcal{L}_{u}+\lambda_{2} \mathcal{L}_{\nabla \mathbf{h}},
\end{equation}

with $\lambda_{1}, \lambda_{2} \in \mathbb{R}_{+}$weighting the importance of the individual loss terms. 
Furthermore, consider two additional loss functions characterizing the satisfaction of Lipschitz bound condition \cite{pauli2021training} and solution completeness condition \eqref{eq: completeness_condition} as

\begin{equation}
    \begin{aligned}
     L_{M}(\theta, \Lambda, \bar{\Lambda}, \bar{\bar{\Lambda}})=-c_{l_{1}} \log \operatorname{det}(M(\theta, \Lambda)) \\ -c_{l_{2}} \log \operatorname{det}(M(\bar{\theta}, \bar{\Lambda}))
      -c_{l_{3}} \log \operatorname{det}(M(\bar{\bar{\theta}}, \bar{\bar{\Lambda}}))
    \end{aligned}
\end{equation}
\begin{equation}
    \begin{aligned}
    L_{v}(\eta)=\max \left(0,\mathcal{L}_{\max } \hat{\epsilon}+\eta\right)
    \end{aligned}
\end{equation}
where $\mathcal{L}_{h}$, $\mathcal{L}_{dh}$ and $\mathcal{L}_{d2h}$ that appear in $M(\theta, \Lambda)$, $ M(\bar{\theta}, \bar{\Lambda)}$ and $ M(\bar{\bar{\theta}}, \bar{\bar{\Lambda)}}$, is used to compute $\mathcal{L}_{\text {max }}$. These parameters, along with $\hat{\epsilon}$, are hyper-parameters that are chosen a priori. Moreover, $c_{l_{1}}, c_{l_{2}}, c_{l_{3}}$ are positive weight coefficients for the sub-loss functions.

% \subsection{Learning the System Dynamics}
% \label{learning system dynamics}
% To learn the system dynamics, we use another neural network parameterized by $\psi$, i.e., $\mathbf{F}(x \mid \psi)$, to estimate both $\Delta \mathbf{f}(x)$ and $\Delta \mathbf{g}(x)$. Using this neural network, our estimated dynamics is defined as

% $$
% \dot{\tilde{x}}(x, u \mid \psi)=\widehat{\mathbf{f}}(x)+\widehat{\mathbf{g}}(x) u+\mathbf{F}(x \mid \psi)\left[\begin{array}{l}
% 1 \\
% u
% \end{array}\right]
% $$

% Common methods in learning the system dynamics require obtaining data of $\dot{x}[23]$ or the next state (i.e., state at the "next" time step) [36]. Using $\dot{x}$ requires additional sensors, e.g., inertial measurement units. Using the next state is also not accurate, since the commonly used integration schemes only approximate the true discrete-time dynamics. Thus, instead of learning the system dynamics via a regression problem on $\dot{x}$ or the next state, we form a regression problem on $\dot{h}(x)$ [32], which is given by

% $$
% \dot{h}(x)=\frac{\partial h(x)}{\partial x}(\mathbf{f}(x)+\mathbf{g}(x) u)
% $$

% Using the estimated dynamics from (28) and the estimated CBF from (19), the estimated $\dot{h}(x)$ is given as

% $$
% \dot{\tilde{h}}(x, u, \theta \mid \psi)=\frac{\partial \tilde{h}(x, \theta)}{\partial x} \dot{\tilde{x}}(x, u \mid \psi)
% $$

% When learning the system dynamics, although the value of $\dot{\tilde{h}}$ does depend on $\theta$, the gradient is only calculated with respect to $\psi$. Therefore, in the remainder of this section, we will omit $\dot{\tilde{h}}$ 's dependency on $u$ and $\theta$. Additionally, we can numerically estimate $\dot{h}(x)$ using the central difference method

% $$
% \widehat{\dot{\tilde{h}}}(x)=\frac{\tilde{h}\left(x_{s}\right)-\tilde{h}\left(x_{u}\right)}{2 \Delta t}
% $$

% where $x_{s}$represents the next state, and $x_{u}$represents the previous state. To learn the weights $\psi$, we use the loss function defined as

% $$
% \mathcal{L}_{\psi}(\psi)=\sum_{x_{i} \in \mathcal{X}_{s} \cup \mathcal{X}_{u}}\left(\hat{\tilde{h}}\left(x_{i}\right)-\dot{\tilde{h}}\left(x_{i} \mid \psi\right)\right)^{2}
% $$

% Note that when performing gradient-based updates for $\psi$, the gradient of $\mathcal{L}_{\psi}$ is only calculated with respect to $\psi$. Given that

% $$
% \lim _{\Delta t \rightarrow 0} \hat{\dot{\tilde{h}}}(x)=\frac{\partial \tilde{h}(x)}{\partial x} \dot{x}
% $$

% we can show that for a small $\Delta t$ and loss value, the error in the learned dynamics is bounded. Assuming the loss is less than some positive value, i.e.,

% $$
% \mathcal{L}_{\psi}(\psi) \leq \epsilon
% $$

% where $\epsilon \in \mathbb{R}_{+}$, yields

% $$
% \hat{\dot{\tilde{h}}}\left(x_{i}\right)-\dot{\tilde{h}}\left(x_{i} \mid \psi\right) \leq \sqrt{\epsilon}
% $$

% Given that the central difference method has a truncation error of $\mathcal{O}\left(\Delta t^{2}\right)$, we have

% $$
% \widehat{\dot{\tilde{h}}}(x)=\frac{\partial \tilde{h}(x)}{\partial x} \dot{x}+\mathcal{O}\left(\Delta t^{2}\right)
% $$

% which leads to

% $$
% \frac{\partial \tilde{h}\left(x_{i}\right)}{\partial x}\left(\dot{x}_{i}-\dot{\tilde{x}}\left(x_{i}, u \mid \psi^{*}\right)\right)+\mathcal{O}\left(\Delta t^{2}\right) \leq \sqrt{\epsilon}
% $$

% Then, we have the following bound on the error of the learned dynamics, i.e., $\dot{x}_{i}-\dot{\tilde{x}}$ :

% $$
% \dot{x}_{i}-\dot{\tilde{x}}\left(x_{i}, u \mid \psi^{*}\right) \leq\left[\frac{\partial \tilde{h}\left(x_{i}\right)}{\partial x}\right]^{\dagger}\left(\sqrt{\epsilon}+\mathcal{O}\left(\Delta t^{2}\right)\right)
% $$

% This shows that with a small enough $\Delta t$ and loss value, our proposed algorithm can learn a reasonably accurate model of the system dynamics.

\subsection{Training Process}
\label{training}
We train $\tilde{h}$ using a supervised learning approach. For supervised learning, one key assumption for the training data is that they are independently and identically distributed (i.i.d). The overall training procedure is as follows. We first fix all the hyper-parameters required for the training, including $\hat{\epsilon}, \mathcal{L}_{h}, \mathcal{L}_{dh}, \mathcal{L}_{d2h}, \lambda_{1}, \lambda_{2}, c_{l_{1}}, c_{l_{2}}, c_{l_{3}}$, and the maximum number of epochs considered. Note that at every epoch, we perform the training over several batches, which is also fixed a priori. This means that the training data sets $\mathcal{S}, \mathcal{U}$ and $\mathcal{E}$ are randomly shuffled into several batches, and the loss is calculated for each batch at a time. At each time step, given the current state, the performance controller computes a potentially unsafe action $u_{\text {ref }}(x)$. Then, the unsafe action is passed through the learned CBF filter, making it the estimated safe action. The learned CBF-QP controller has the form


\begin{equation}
    \begin{aligned}
        \min _{u \in \mathcal{U}} & \left\|u-u_{\text {ref }}(x)\right\| \\
        \quad & \textrm{s.t.} \frac{\partial \tilde{h}\left(x_{i} \mid \theta\right)}{\partial x} (\mathbf{f}(x)+\mathbf{g}(x) u)  + \frac{1}{2}tr(\sigma^\intercal \frac{\partial^2 \tilde{h}\left(x_{i} \mid \theta\right)}{\partial x^2} \sigma) \\
        & \geq-\alpha(\tilde{h}(x))
    \end{aligned}
\end{equation}


Finally, the control action $u$ is applied to the environment. Additionally, the current state, the learned CBF, and the estimated safe action are stored in the corresponding replay buffer at each time step. After each episode ends, data sampled from the replay buffer are used to compute the loss functions. Then, using a stochastic gradient descent algorithm, e.g., ADAM, the weights of the two networks $ \tilde{h}$ is updated. This procedure is repeated until the network converges or if a predefined maximum episode number is reached. For our proposed approach, all of the learning is done offline in a simulation environment. After the learning process converges, the learned CBF-QP can then be deployed to the intended system.

==> problem_formulation.tex <==
In this study, we express the $\mathrm{CBF}$ using neural networks and conduct training with a finite set of data samples. Formal guarantees for its correctness under stochastic conditions across the entire state set are provided, incorporating a validity condition. This section is dedicated to outlining the derivation of the validity condition, a crucial component in our proposed training framework. It is essential to note that we assume the availability of pre-existing neural network candidates corresponding to CBF, specifically denoted as $\tilde{h}(x \mid\theta)$, where $\theta$ represents the network's weights. We employ scenario-based verification techniques to establish the validity condition, which assesses whether the CBF meets the criteria outlined in equations \eqref{eq:setc1}, \eqref{eq:setc2}. To achieve this, we reframe these conditions initially as a robust convex problem (RCP):
\begin{equation}\label{eq: rcp}
    \mathrm{RCP}: \begin{cases}\min _{\eta} & \eta \\ \text { s.t. } & \max \left(q_{k}(x)\right) \leq 0, k \in\{1,2,3\} \\ & \forall x \in X, \eta \in \mathbb{R}\end{cases}
\end{equation}

where
\begin{equation} \label{eq:q_conditions}
    \begin{aligned}
        & q_{1}(x)=\left(-\tilde{h}(x \mid \theta)-\eta\right) \mathbbm{1}_{X_{s}}, \\
        & q_{2}(x)=\left(-\tilde{h}(x \mid \theta)+\varepsilon-\eta\right) \mathbbm{1}_{X_{u}}, \\
        & q_{3}(x)=\frac{\partial \tilde{h}\left(x_{i} \mid \theta\right)}{\partial x} \dot{x} +\frac{1}{2}tr(\sigma^\intercal \frac{\partial^2 \tilde{h}\left(x_{i} \mid \theta\right)}{\partial x^2} \sigma) \\
        & +  \alpha\left(\tilde{h}\left(x_{i} \mid \theta\right)\right)-\eta,
    \end{aligned}
\end{equation}

where $\varepsilon$ is a small positive value to ensure the strict inequality. Let the optimal solution of the RCP be $\eta_{\mathrm{RCP}}^{*}$. Then, if $\eta_{\mathrm{RCP}}^{*} \leq 0$, then the satisfaction of conditions (6)-(8) implies the satisfaction of conditions (2)(4), and the neural network-based $\tilde{h}(x \mid \theta)$ is valid. However, finding a solution to the RCP is not possible due to function $f$ in (8) being unknown. To circumvent this, one can take a sampling based approach by appropriately selecting $N$ data samples from the state set $X$, and then reformulating the $\mathrm{RCP}$ in \eqref{eq: rcp} into a scenario convex problem (SCP). We obtain the data as follows. First, cover sets are constructed for $X, X_{s}$ and $X_{u}$, respectively. Cover of a set $X$ (resp. $X_{s}, X_{u}$ ) is a set consisting of subsets of $X$ (resp. $X_{s}, X_{u}$ ) whose union equals $X$ (resp. $X_{s}, X_{u}$ ). The cover sets are constructed such that they consist of hyper-rectangles
\begin{equation}
    H_{i}\left(x, \epsilon_{i}\right):=\left\{x \in X \mid-\epsilon_{i} \leq x-x_{i} \leq \epsilon_{i}\right\},
\end{equation}
centered at grid points $x_{i} \in X, i \in\{1, \ldots, N\}$, with $\epsilon_{i} \in \mathbb{R}^{n}$. Now, consider $\hat{\epsilon}=\max _{i}\left\|\epsilon_{i}\right\|$. Then, for any $x \in X$ (resp. $X_{0}, X_{u}$ ), there exists $x_{i}, i \in\{1, \ldots, N\}$, such that $\left\|x-x_{i}\right\| \leq \hat{\epsilon}$. The data sets $\mathcal{S}, \mathcal{U}$ and $\mathcal{E}$ corresponding to the safe set $X_{s}$, unsafe set $X_{u}$, and state set $X$, respectively, are then obtained by considering the representative points $x_{i}$, for all $i \in\{1, \ldots, N\}$, as

\begin{equation}\label{eq: SUE}
    \begin{aligned}
        & \mathcal{S}=\left\{x_{i} \mid x_{i} \in X_{s}, \forall i \in\{1, \ldots, N\}\right\}, \\
        & \mathcal{U}=\left\{x_{i} \mid x_{i} \in X_{u}, \forall i \in\{1, \ldots, N\}\right\}, \text { and } \\
        & \mathcal{E}=\left\{x_{i} \mid \forall i \in\{1, \ldots, N\}\right\}
    \end{aligned}
\end{equation}

Utilizing these sets, we construct a scenario convex problem (SCP), defined as follows:

\begin{equation}\label{eq: scp}
    \mathrm{SCP}: \begin{cases}\underset{\eta}{\min } & \eta \\ \text { s.t. } & q_{1}\left(x_{i}\right) \leq 0, \forall x_{i} \in \mathcal{S}, \\ & q_{2}\left(x_{i}\right) \leq 0, \forall x_{i} \in \mathcal{U}, \\ & q_{3}\left(x_{i}\right) \leq 0, \forall\left(x_{i}, f\left(x_{i}\right)+ g\left(x_{i}\right)u_{i}\right) \in \mathcal{E}, \\ & \eta \in \mathbb{R}, i \in\{1, \ldots, N\},\end{cases}
\end{equation}

where $q_{k}(x), k \in\{1,2,3\}$ are defined as in \eqref{eq:q_conditions}. Since there are finitely many data samples $x_{i}$, and SCP is a linear program with respect to the decision variable $\eta$, finding a solution to the SCP is tractable. Let the optimal solution of the SCP be $\eta^{*}$. Now we want to prove that $\eta^{*}$ is also a feasible solution to the original RCP \eqref{eq: rcp}. To do so, one must utilize a Lipschitz continuity assumption on the system as well as conditions \eqref{def:positive-invariance}.

\begin{theorem}\label{thm: }{\it
Consider a continuous time control system, and safe and unsafe sets $X_{s} \subseteq X$ and $X_{u} \subseteq X$, respectively. Let  $\tilde{h}(x \mid \theta)$ be the neural network-based CBF. For the SCP \eqref{eq: scp} constructed by utilizing $N$ samples as given in equations \eqref{eq: SUE}, let $\eta^{*}$ be the optimal value. Then $\tilde{h}(x \mid \theta)$ is a valid CBF, i.e., they satisfy conditions \eqref{eq:setc1}\eqref{eq:setc2}, if the following condition holds:}
\begin{equation} \label{eq: completeness_condition}
    \mathcal{L}_{\max } \hat{\epsilon}+\eta^{*} \leq 0
\end{equation}
\end{theorem}

\begin{proof}
% The probabilistic relation between the optimal values of RCP and SCP is  given by \cite{}:
% \begin{equation}
%     \mathbb{P}^N \{ \eta_{RCP}^{*} - \eta_{SCP}^{*}\leq \mathcal{L}_{\max}\hat{\epsilon}\} \geq 1 - \beta
% \end{equation}

\end{proof}

==> sections/introductionV2.tex <==


In the rapidly evolving landscape of control theory, ensuring safety in real-world applications has emerged as a paramount concern. With the pervasive integration of automated systems such as self-driving cars, the ability to guarantee their safety becomes increasingly critical. Current methods, including traditional optimal control approaches and Hamilton-Jacobi reachability analysis, have been instrumental in addressing safety requirements by casting them as constraints or generating safe controls offline. However, the scalability limitations of these methods, coupled with the challenge of swift reactions in complex environments, underscore the need for alternative approaches to safety assurance.
With the rise in popularity of learning-based methods in control synthesis, learning-based methods have also been used to synthesize controllers for safety-critical tasks. However, most learning-based methods require a significant amount of unsafe interactions to learn a safe controller, which might be costly or impossible to obtain.

One promising avenue in addressing safety concerns is through the utilization of Control Barrier Functions (CBFs) \cite{Ames_2017}\cite{8796030}. CBFs serve as a practical method for synthesizing safe control by acting as a safety filter for potentially unsafe performance controllers. By formulating controllers through Quadratic Programs (QPs), solvable at high frequencies with modern optimization solvers, CBFs have found applications in various safety-critical tasks, including bipedal~\cite{ames} and quadrupedal locomotion, adaptive cruise control, and multi-agent aerial maneuvers. However, traditional methods for identifying valid CBFs face challenges, particularly with nonlinear or nonconvex constraints, necessitating the exploration of alternative approaches to ensure the efficacy of CBFs in guaranteeing safety.

In recent years, the emergence of neural network-based safety certificate synthesis has garnered considerable attention as a potential solution to the limitations of classical approaches. By parameterizing formulations as neural networks, the need for a mathematical model is circumvented, offering greater flexibility and adaptability in addressing safety specifications. However, this approach introduces its own set of challenges, as neural network-based formulations lack formal guarantees and may not satisfy conditions across the entire state set due to finite training samples. Thus, while neural network-based CBFs hold promise in enhancing safety assurance, further exploration and development are needed to address their current limitations and ensure their applicability in safety-critical systems.

% However, a major caveat of the aforementioned approach is that it requires mathematical knowledge about the system in the form of a model. Since precise mathematical models are not always available due to large complexity of the systems, one needs to consider alternative model-free approaches. Another drawback of the approach is the difficulty in searching for suitable CBFs. In general, one requires to find an appropriate and valid CBF

% In recent year learning based controllers have shown great promise, but there are no safety guarantees, thus making it hard to be applied for safety-critical applications.

%  In recent years, the development of machine learning (ML) has created unprecedented opportunities to control modern autonomous systems with growing complexity.

%  There is some existing work, that synthesises a CBF using neural networks but they lack the completeness guarantees. There is also some work on the synthesis of safe controller using neural network based control barrier certificates (CBC) in discrete time setting along with the completeness guarantee. 

%  In this work, we present a 


%  Ensuring safety is crucial when designing controllers for real-world applications. With the increasing usage of automated systems, e.g., self-driving cars, the ability to guarantee the safety of such systems becomes increasingly important. In optimal control, safety is often ensured by casting the safety requirements as constraints. However, when the optimization problem gets larger, the solution time increases rapidly, limiting its usage for guaranteeing safety in complex environments, which usually requires the control system to react quickly. Recently, Hamilton-Jacobi reachability analysis has been used to generate safe controls. When solved offline, it provides a way to generate safe controls quickly online. However, its usage is greatly limited by the curse of dimensionality. With the rise in popularity of learning-based methods in control synthesis, learning-based methods have also been used to synthesize controllers for safety-critical tasks. However, most learning-based methods require a significant amount of unsafe interactions to learn a safe controller [28], which might be costly or impossible to obtain.

% Another popular method to synthesize safe control is utilizing control barrier functions (CBFs). CBFs can be used as a safety filter for an unsafe performance controller. The controller can be obtained by solving a quadratic program (QP) which can be done at a very high frequency using modern optimization solvers. Given its many advantages, CBFs have been used on many safety-critical tasks, e.g., biped and quadrupedal locomotion on stepping stones [26] [16], adaptive cruise control [2], and multi-agent aerial maneuver [29].

% Although CBF provides a promising direction in safe controller synthesis, we need to have the access to a valid $\mathrm{CBF}$. A common approach to finding a valid CBF is to start with a description of the safe set, usually in the form of state constraints, and find a function that is positive only within the safe set and has the appropriate relative degree with respect to the system dynamics. This method is plausible for simple constraints. However, finding a valid CBF that recovers the entire safe set becomes increasingly challenging as the constraints become nonlinear or nonconvex. To mitigate this issue, work has been done in learning the CBF. In [31], human demonstrations have been used to map the boundaries of the safe set, and a CBF is then learned. This method may not scale to constraints in higher dimensions. Instead of having information on safe set boundaries, work has been done on utilizing expert demonstrations of safe and unsafe trajectories [30]. Additionally, work has been done in learning CBFs using data collected online. In [22], a $\mathrm{CBF}$ is synthesized using only onboard sensors. Recently, work has been done in learning a CBF starting from an initial conservative CBF. In [34], an $\mathrm{HCBF}$ is used to warm start a dynamic program that refines the HCBF to enlarge the recovered safe set. In [12], a learning-based approach is used to learn the difference between a conservative $\mathrm{HCBF}$ and a $\mathrm{CBF}$ that recovers a more significant portion of the safe set.


% Formal verification and synthesis of complex systems against safety specifications is of utmost importance in the field of control theory, especially due to the emergence of safety-critical applications such as autonomous vehicles, drones, robots, medical devices, etc. Methods utilizing control barrier functions (CBFs) provide an effective mechanism to formally generate controllers enforcing the satisfaction of safety specifications. In particular, control barrier functions are real-valued functions defined over the state set of the system. They act as a barrier between the safe and unsafe regions, providing sufficient conditions such that the barrier is never crossed by the closed-loop system trajectories. However, a major drawback of this approach is the difficulty in finding a suitable $\mathrm{CBF}$ especially for large complex systems.

% Neural network-based safety certificate synthesis has gained considerable attention recently (Dawson et al., 2023) since it has great potential to alleviate the issues concerning model-based one. First, neural network training is completely data-driven. Therefore, by parameterizing CBFs as neural networks, one avoids the requirement of a mathematical model. Second, neural networks are capable of approximating any continuous function (Barron, 1994). However, CBFs based on neural networks lack formal guarantees and cannot be applied to safety-critical systems without further verification. This is due to the fact that neural networks are trained on a finite number of samples from the state set, and as a result, the trained networks are not guaranteed to satisfy the required $\mathrm{CBF}$ conditions over the entire state set (i.e. unseen samples from the state set). Therefore, one is required to formally verify the trained CBFs post facto to ensure safety.

\subsection{Related Work}

Barrier certificates for safe control were first proposed in \cite{prajna2007framework}. More recently, CBFs have emerged as promising approaches to safe control, due to their compatibility with a wide variety of control laws. For control systems with polynomial dynamics, CBFs can be synthesized by solving sum-of-squares (SOS) optimization programs \cite{clark2021verification,clark2022semi,kang2023verification,dai2023convex}. 
Polynomial CBFs are limited in applications due to the limitation of the template and function space \cite{anand2023formally}. 
To overcome the shortcomings of CBF synthesis using SOS-based approaches, neural control barrier functions (NCBFs) \cite{dawson2022safe,dawson2023safe,liu2023safe,9993334, dai2023learning}, which represent CBFs using neural networks, are developed.
Recent research shows great promise of neural barrier functions in flexibility in configuring complex environments and potential to scale up. 
NCBFs leverage the universal approximation power of neural networks \cite{tabuada2022universal,hornik1989multilayer,csaji2001approximation}, facilitating the CBF synthesis.
A class of recent neural barrier certificate is to construct a nominal control policy and prove that it satisfies the NCBF constraints, including SMT-based methods~\cite{zhao2020synthesizing,abate2021fossil,abate2020formal}, mixed integer programs \cite{zhao2022verifying} and nonlinear programs \cite{NEURIPS2023_120ed726}.
\textcolor{blue}{[details on related work on neural control barrier certificate]}
Existing works focused on certificating deterministic systems and joint synthesis of safe control policy \cite{jin2020neural}. However, safety verification of stochastic systems are less explored. 

% \cite{10.1145/3447928.3456638} \cite{10066195} \cite{10.1007/978-3-030-72016-2_20} \cite{9157966} \cite{9990576}

\subsection{Contributions}
In this paper, we study the synthesis of stochastic neural CBF. 
We consider a continuous-time stochastic nonlinear control-affine system. 
% We derive the sufficient condition for the safety of SNCBF-based system. 
We construct a sample-based training framework to train Stochastic NCBF (SNCBF) and prove the trained SNCBF ensuring efficacy across the entire state space with only a finite number of data points. To summarize, this paper makes the following contributions.
\begin{itemize}
    \item We propose a training framework to synthesize provably correct Control Barrier Functions (CBFs) parameterized as neural networks for continuous-time, stochastic systems eliminating any need for post hoc verification.
    \item Our methodology establishes completeness guarantees by deriving a validity condition, ensuring efficacy across the entire state space with only a finite number of data points. We train the network by enforcing Lipschitz bounds on the neural network, its Jacobian and Hessian terms.
    \item We evaluate our approach using two case studies on the limited stable region problem of an inverted pendulum. We show that our training framework successfully construct a SNCBF. \textcolor{blue}{(description on the result of our proposed method)}
\end{itemize}

\subsection{Organization}
The rest of this paper is organized as follows. Preliminaries explaining the concept of control barrier functions (CBFs) and safety filter designs are introduced in Section \ref{section: Background}. Problem formulation is discussed in Section \ref{section: Problem Formulation}. The method proposed to synthesize the CBFs using neural networks, the construction of loss functions and algorithm to train it, is discussed in Section \ref{section: Method}. The simulation results will be discussed in Section \ref{section: Simulation}. Finally, we present our conclusion in Section \ref{section: Conclusions}. 



% $<.\:,\:.>$ denotes the inner product of two vectors.
% $\hat{i}$ and $\hat{j}$ stands for unit vectors along x-axis and y-axis respectively. The units used in the simulations are SI units.

==> sections/sim_resultsV2.tex <==
In this section, we evaluate our proposed approach using an inverted pendulum model \textcolor{blue}{[reference]}. All experiments are are conducted on a PC with an Intel i7-7800X CPU, 32GB RAM and NVIDIA GeForce RTX 3090 GPU. 

\subsection{Inverted Pendulum}
We consider a continuous time stochastic inverted pendulum dynamics given as follows:
\begin{equation}
    d\left[\begin{array}{l}
    \theta \\
    \dot{\theta}
    \end{array}\right]=(\left[\begin{array}{c}
    \dot{\theta} \\
    \frac{g}{l}\sin(\theta)
    \end{array}\right]+\left[\begin{array}{c}
    0 \\
    \frac{1}{m l^{2}} 
    \end{array}\right] u) dt + \sigma \ dW_{t}
\end{equation}

where $\theta \in \mathbb{R}$ denotes the angle, $\dot{\theta} \in \mathbb{R}$ denotes the angular velocity, $u \in \mathbb{R}$ denotes the controller, $m$ denotes the mass and $l$ denotes the length of the pendulum. We let the mass $m= 1$kg, length $l=10$m and the disturbance $\sigma = [0.1, 0.1]^T$

The inverted pendulum operate in a state space given as $X=\left[-\frac{\pi}{4}, \frac{\pi}{4} \right]^{2}$. 
The system is required to stay in a limited stable region.  
The initial safe region is given as $X_{s}=\left[-\frac{\pi}{15}, \frac{\pi}{15}\right]^{2}$ and the unsafe region is given as $X_{u}=X \backslash \left[-\frac{\pi}{6}, \frac{\pi}{6}\right]^{2}$. 

We assume that the model is known. We then train the SNCBF. The SNCBF $\tilde{h}$ consists of one hidden layer of $20$ neurons, with Softplus activation function ($log(1+exp(x)$). 

\begin{figure}[t]
    \centering
\vspace{-0.6em}
\includegraphics[width=0.8\linewidth]{images/barr_plot.png}
\vspace{-0.6em}
    \caption{Plot of $\tilde{h}\left(x \mid \theta\right)$ over $X$. Blue and red regions denote the safe region ($\tilde{h} \geq 0$) and the unsafe region ($\tilde{h} < 0$), respectively. The initial safety region boundary and unsafe region boundary is denoted by black boxes. We observe that the boundary of trained SNCBF (black dots) successfully separate the unsafe and safe region. }
    \label{fig:2d_sample}
\end{figure}

\begin{figure}[t]
    \centering
\vspace{-0.6em}
\includegraphics[width=0.9\linewidth]{images/3D_plot.png}
    \caption{3D Plot of $\tilde{h}\left(x \mid \theta\right)$ over $X$. We observe that the safe region is greater than zero while unsafe region has negative function value. }
    \label{fig:3d_sncbf}
\end{figure}
We first fix the training hyper-parameters $\bar{\epsilon}=0.00016$, $L_{h} = 0.01$, $L_{dh} = 0.4$ and $L_{d2h} = 2$. Then, we compute $L_{\max} = 2.4$. We perform the training to simultaneously minimize the loss functions $\mathcal{L}_{\theta}, \mathcal{L}_{M}$, and $\mathcal{L}_{v}$. The training algorithm then converges to obtain the CBF $\tilde{h}\left(x \mid \theta\right)$ along with $\psi^{*}=-0.00042$. 
The trained SNCBF is visualized in both 2D with sample points in Fig. \ref{fig:2d_sample} and in 3D function value heat map in Fig. \ref{fig:3d_sncbf}. As shown in Fig. \ref{fig:2d_sample}, the trained SNCBF successfully separate the initial safety region boundary and unsafe region boundary denoted by black boxes. In Fig. \ref{fig:3d_sncbf}, we observe that the safe region is greater than zero while unsafe region has negative function value, which shows the trained SNCBF has correct value.
Using Theorem \ref{thm: }, we can verify that the SNCBF thus obtained is valid, thus ensuring safety. 

\subsection{Obstacle Avoidance}

We consider an autonomous mobile robot navigating on a road following the dynamics \cite{dubins1957curves} given below
\begin{equation*}
    \dot{x} = f(x) + g(x)u,
\end{equation*}

where $x:=[x_1, x_2, \psi]^T\in\mathcal{X}\subseteq\mathbb{R}^3$ is the state consisting of the location $(x_1,x_2)$ of the robot and its orientation $\psi$, $u$ is the input that controls the robot's orientation, $f(x) = [\sin\psi,\cos\psi,0]^T$, and $g(x)=[0,0,1]^T$.

The mobile robot is required to stay in the road while avoid pedestrians sharing the field of activities. 
We set the location of the pedestrian as $(0,0)$.
Then the safety region is formulated as $\mathcal{C} = \left\{\mathbf{x} \in \mathcal{X}: x_1^2+x_2^2 \geq 0.04, \text{ and } x_2 \geq -0.3\right\}$, where $\mathcal{X}= [-2,2]^3$.



==> sim_results.tex <==
In this section, we evaluate our proposed approach using an inverted pendulum model \textcolor{blue}{[reference]}. All experiments are are conducted on a PC with an Intel i7-7800X CPU, 32GB RAM and NVIDIA GeForce RTX 3090 GPU. 

The SNCBF $\tilde{h}$ consists of one hidden layer of $20$ neurons, with Softplus activation function ($log(1+exp(x)$).
We consider a continuous time stochastic inverted pendulum dynamics given as follows:
\begin{equation}
    d\left[\begin{array}{l}
    \theta \\
    \dot{\theta}
    \end{array}\right]=(\left[\begin{array}{c}
    \dot{\theta} \\
    \frac{g}{l}\sin(\theta)
    \end{array}\right]+\left[\begin{array}{c}
    0 \\
    \frac{1}{m l^{2}} 
    \end{array}\right] u) dt + \sigma \ dW_{t}
\end{equation}

where $\theta \in \mathbb{R}$ denotes the angle, $\dot{\theta} \in \mathbb{R}$ denotes the angular velocity, $u \in \mathbb{R}$ denotes the controller, $m$ denotes the mass and $l$ denotes the length of the pendulum. The domain is given as $X=\left[-\frac{\pi}{4}, \frac{\pi}{4} \right]^{2}$, the initial safe set is $X_{s}=\left[-\frac{\pi}{15}, \frac{\pi}{15}\right]^{2}$, and the unsafe set as $X_{u}=X \backslash \left[-\frac{\pi}{6}, \frac{\pi}{6}\right]^{2}$, $m= 1$kg, $l=10$m and $\sigma = [0.1, 0.1]^T$. We assume that the model is known. 
\begin{figure}[t]
    \centering
\vspace{-0.6em}
\includegraphics[width=0.8\linewidth]{images/barr_plot.png}
\vspace{-0.6em}
    \caption{Plot of $\tilde{h}\left(x \mid \theta\right)$ over $X$. Blue and red regions denote the safe region ($\tilde{h} \geq 0$) and the unsafe region ($\tilde{h} < 0$), respectively.}
\end{figure}

\begin{figure}[t]
    \centering
\vspace{-0.6em}
\includegraphics[width=0.9\linewidth]{images/3D_plot.png}
    \caption{3D Plot of $\tilde{h}\left(x \mid \theta\right)$ over $X$.}
\end{figure}
We first fix the training hyper-parameters $\bar{\epsilon}=0.00016$, $L_{h} = 0.01$, $L_{dh} = 0.4$ and $L_{d2h} = 2$. Then, we compute $L_{\max} = 2.4$. We perform the training to simultaneously minimize the loss functions $\mathcal{L}_{\theta}, \mathcal{L}_{M}$, and $\mathcal{L}_{v}$. The training algorithm then converges to obtain the CBF $\tilde{h}\left(x \mid \theta\right)$ along with $\psi^{*}=-0.00042$. Using Theorem \ref{thm: }, we can verify that the SNCBF thus obtained is valid, thus ensuring safety. 

